Analyzing the Impact of Splicing Artifacts in Partially Fake Speech Signals

Speech deepfake detection has recently gained significant attention within the multimedia forensics community. Related issues have also been explored, such as the identification of partially fake signals, i.e., tracks that include both real and fake speech segments. However, generating high-quality spliced audio is not as straightforward as it may appear. Spliced signals are typically created through basic signal concatenation. This process could introduce noticeable artifacts that can make the generated data easier to detect. We analyze spliced audio tracks resulting from signal concatenation, investigate their artifacts and assess whether such artifacts introduce any bias in existing datasets. Our findings reveal that by analyzing splicing artifacts, we can achieve a detection EER of 6.16% and 7.36% on PartialSpoof and HAD datasets, respectively, without needing to train any detector. These results underscore the complexities of generating reliable spliced audio data and lead to discussions that can help improve future research in this area.

==> 2_analysis_old.tex <==
\section{Discontinuities and Spectral Leakage}
\label{sec:analysis}

In this paper, we consider the problem of spectral artifacts that may arise when concatenating audio tracks and investigate if these are present in partially fake speech signals.
We start by introducing the concepts of \textit{spectral leakage} and \textit{splicing artifact} and demonstrate how they occur with examples involving the concatenation of simple sinusoids.
This initial, straightforward analysis allows us to thoroughly understand the problem at hand and allows us to make considerations that can then be extended to more complex signals, i.e., speech tracks.

\vspace{0.5em}
\noindent
\textbf{Spectral Leakage.}
A spectral leakage is a phenomenon observed in the frequency domain analysis when energy from a signal spreads across multiple frequency bins.
This effect occurs when analyzing a signal using a Fourier transform, under the incorrect assumption that the signal is periodic within the observation window.
This situation can happen in two distinct scenarios: (a) the signal is periodic, but the length of the window length is not an integer multiple of its period, and (b) the signal is non-periodic.
The mismatch between the actual signal and the assumed periodic model results in a distortion of the frequency spectrum, causing energy to spread across frequency bins that would ideally have zero energy.

To formally explain the occurrence of spectral leakage, let us consider a continuous signal $y_\text{w}(t)$, which is a segment extracted from a longer signal $y(t)$.
This portion is obtained by multiplying $y(t)$ with a rectangular window function $w(t)$, such as
\begin{equation}
y_\text{w}(t) = y(t) \cdot w(t) .
\end{equation}
The rectangular window $w(t)$ is defined as
\begin{equation}
w(t) = \begin{cases} 
1 & \text{if } 0 \le t < T, \\
0 & \text{otherwise},
\end{cases}
\label{eq:rect_window}
\end{equation}
where $T$ represents its time duration.
We can define the Fourier transform of $y_\text{w}(t)$ as
\begin{align}
Y_\text{w}(f) = & \mathcal{F}\{y_\text{w}(t)\} = \mathcal{F}\{y_\text{w}(t) \cdot w(t)\} = \\
= &  Y(f) * W(f) ,
\end{align}
where the ``$*$'' operator indicates convolution, while $Y(f) = \mathcal{F}\{y(t)\}$ and $W(f) = \mathcal{F}\{w(t)\}$ are the Fourier transforms of the original signal $y(t)$ and the window function $w(t)$, respectively.
In particular, when $w(t)$ is defined as in \cref{eq:rect_window}, its Fourier transform is equal to
\begin{equation}
W(f) = T \cdot \text{sinc}(Tf) = T \cdot \frac{\sin(\pi Tf)}{\pi Tf} .
\end{equation}
The presence of the $\text{sinc}$ function introduces sidelobes in the frequency domain, resulting in the spreading of energy across adjacent frequency bins, which is known as spectral leakage.

In the digital domain, when dealing with discrete-time signals, we can minimize the spectral leakage by selecting an analysis window whose length is a multiple of the signal's period. 
This alignment ensures that the signal is sampled at the zero crossing points of the $\text{sinc}$ function, thereby reducing leakage.
Additionally, incorporating multiple signal periods within the window enhances the frequency resolution of the analysis.  
However, when a signal is observed within a finite window with aperiodic boundary conditions, sidelobes appear in the frequency spectrum.
This occurs because the sinc function is no longer sampled at its zero-crossings.
In the time domain, if the analysis window does not capture a periodic segment of the initial signal, the reconstruction of the waveform by re-combining the signal windows will result in sharp transitions, or transients, at the boundaries where the segments join.
These discontinuities lead to frequency smearing in the spectrum, which is challenging to mitigate. This arises because discontinuities in the time domain resemble impulses, which have a flat spectrum in the frequency domain, i.e., contain all frequency components with equal amplitude.
\Cref{fig:pure_sin} shows an example of this effect.

\begin{figure*}[t]
\centering
\includegraphics[width=.95\textwidth]{Images/pure_sin.pdf} 
\caption{Frequency domain analysis of a sinusoid. $f_\text{s}$ = \SI{16}{\kilo\hertz}, $f_0$ = \SI{800}{\hertz}, \num{20} samples per period.
Left: FFT up to Nyquist. Center: Magnitude Spectrogram (up to 4000 Hz). Right: Spectrogram (dB).
Top: STFT window of \num{80} samples (multiple of the period). Bottom: STFT window of \num{88} samples (not a multiple of the period), with spectral artifacts.}
\label{fig:pure_sin}
\end{figure*}

\vspace{0.5em}
\noindent
\textbf{Splicing Artifact.}
Spectral leakage is a well-known issue in signal processing.
To mitigate it, alternative window functions such as Hamming or Hanning windows can be employed during analysis. These functions gradually reduce the signal amplitude towards the window edges, smoothing the spectral transitions and reducing spectral leakage compared to the abrupt cutoff of a rectangular window.
Nevertheless, if we are presented with a spliced signal that already contains a discontinuity, taking a \gls{stft} will reveal it regardless of our choice of parameters. 

A spliced signal can be formally defined as follows.
Let us consider two discrete-time signals $\mathbf{x}_1(n)$ and $\mathbf{x}_2(n)$, with length $N_1$ and $N_2$, sampled at the same sampling frequency $f_\text{s}$. We define the spliced audio track $\mathbf{x}_\text{s}(n)$ as the concatenation in time of $\mathbf{x}_1(n)$ and $\mathbf{x}_2(n)$, such as 
\begin{equation}
	\mathbf{x}_\text{s}(n) = [\mathbf{x}_1(n), \mathbf{x}_2(n)] .
\end{equation}
The resulting length of $\mathbf{x}_\text{s}$ is $N = N_1 + N_2$, and the splicing point as the sample where the two signals join, specifically at $N_1 + 1$.
Let us assume an elementary spliced signal $\mathbf{x}$ as an example, where a sinusoid $\mathbf{x}_1 = \sin(n)$ is concatenated with a shifted copy of itself $\mathbf{x}_2 = \sin(n + \pi)$. 
Even if we pick an analysis window equal to $k \times 2\pi$, i.e., a multiple of the period of the original sinusoid, the abrupt transition will cause leakage in the spectrum at the concatenation point.
In this work, we refer to this particular type of spectral leakage as splicing artifact.

An example of this phenomenon is illustrated in the first column of \cref{fig:discontinuity}. 
In this case, given that the signal is predominantly sinusoidal, the issue can be mitigated by prioritizing frequency resolution over time resolution, considering the longest possible analysis window. 
This approach would enable the \gls{stft} to neglect a punctual temporal analysis, therefore reducing the impact of the discontinuity, as shown by the horizontal progression in \cref{fig:discontinuity}.
However, for more complex signals such as speech, which contain a broad spectrum of frequency components, it is essential to find a balance between time and frequency resolution to represent the signal accurately.
This means that if malicious users aim to create spliced tracks that do not contain any splicing artifact, they must implement a mitigation strategy at the synthesis stage to address these issues.
It is important to note that although this study focuses on partially fake speech, these considerations apply to any signal regardless of whether the source samples are authentic or synthetically generated.

\begin{figure*}
\centering
\includegraphics[width=\textwidth]{Images/disc_freq_res.pdf} 
\caption{Frequency domain analysis of a sinusoid concatenated with a copy of itself shifted by $\pi$. $f_\text{s}$ = \SI{16}{\kilo\hertz}, $f_0$ = \SI{4000}{\hertz}, \num{4} samples per period in the original sinusoid. STFT windows in samples from left to right: \num{40}, \num{160}, \num{260}, \num{388}. Spectrograms in dBs.}
\label{fig:discontinuity}
\end{figure*}

\iffalse

In this paper, we consider the problem of partially fake speech signals and analyze the spectral artifacts that may arise in correspondence with their splicing point.
Let us consider a discrete-time input speech signal $\mathbf{x}$ sampled with a sampling frequency $f_\text{s}$.
We consider the signal $\mathbf{x}$ as belonging to a class $y_\text{S} \in \{0, 1 \}$, where \num{1} indicates that $\mathbf{x}$ is spliced, while \num{0} indicates that it is not.
We call a signal $\mathbf{x}$ as spliced when it has been obtained by the concatenation in time of two shorter signals $\mathbf{x}_1$ and $\mathbf{x}_2$.
% say that we can also define the class $y_\text{C}$ of each sub-track, being it real or fake
% when two tracks concatenated together belong to two different classes $y_\text{C}$, we have a partially fake speech signal
% talk about the splicing point, which is the point where the two tracks are concatenated
% say that artifacts may arise in correspondence of the splicing point
\fi
